Non-Orthogonal Multiple Access Assisted by Reconfigurable Intelligent Surface Using Unsupervised Machine Learning

Nonorthogonal multiple access (NOMA) with multi-antenna base station (BS) is a promising technology for next-generation wireless communication, which has high potential in performance and user fairness. Since the performance of NOMA depends on the channel conditions, we can combine NOMA and reconfigurable intelligent surface (RIS), which is a large and passive antenna array and can optimize the wireless channel. However, the high dimensionality makes the RIS optimization a complicated problem. In this work, we propose a machine learning approach to solve the problem of joint optimization of precoding and RIS configuration. We apply the RIS to realize the quasi-degradation of the channel, which allows for optimal precoding in closed form. The neural network architecture RISnet is used, which is designed dedicatedly for RIS optimization. The proposed solution is superior to the works in the literature in terms of performance and computation time.

==> motivation.tex <==
\section{Machine Learning Solution for Joint Precoding and RIS Configuration}
\label{sec:ml}

% \subsection{Motivation and Framework of Machine Learning Enabled RIS in NOMA}
% \label{sec:motivation}
% \subsubsection{Motivation of applying RIS to NOMA}
% The performance of \gls{noma} depends heavily on the channel for two reasons.
% 1) 
% According to Section~\ref{sec:quasi},
% a prerequisite to apply the optimal precoding \eqref{eq:optimal_precoding1} and \eqref{eq:optimal_precoding2} is the quasi-degradation of the channel~\eqref{eq:quasi_degradation}.
% 2) Among the quasi-degraded channels,
% more advantageous channels (e.g., with higher channel gains) are able to realize a lower transmission power subject to the rate requirements.
% These two considerations imply that the \gls{ris} can be a good company to \gls{noma} because its ability to make a channel quasi-degraded and to optimize the quasi-degraded channel for a lower transmission power.

\subsection{Framework of Unsupervised Machine Learning for RIS Optimization}
% Although the application of \gls{ris} to \gls{noma} seems promising,
% the complicated problem formulation and precoding as well as the high dimensionality of the optimization problem due to the large number of \gls{ris} antennas
% makes the problem very difficult and time-consuming to solve with analytical methods.
In this work, we propose to solve the problem with an unsupervised machine learning approach to optimize the \gls{ris} configuration.

We define a neural network $N_\theta$,
which is a function parameterized by $\theta$ and
maps from the channel feature $\boldsymbol{\Gamma}$
(the channel feature is a formatted representation of the channel gains appeared in \eqref{eq:channel},
as will be defined in detail in Section~\ref{sec:feature_definition})
to the \gls{ris} phase shifts $\boldsymbol{\Phi}$,
i.e.,
\begin{equation}
\boldsymbol{\Phi} = N_\theta(\boldsymbol{\Gamma}).
\label{eq:nn}
\end{equation}
% Thanks to the flexibility of the neural network,
% $N_\theta$ can realize complicated mappings that are difficult or even impossible to be expressed analytically.
With the optimal precoding for quasi-degraded channels presented in Section~\ref{sec:quasi},
% the precoding vectors are fully determined by the channel feature.
our objective function $L$ (including the transmission power $P$ and a penalty term to force quasi-degradation,
as will be defined in Section~\ref{sec:objective})
is fully determined by the channel feature $\boldsymbol{\Gamma}$ and the \gls{ris} configuration $\boldsymbol{\Phi}$.
We can write the objective as
\begin{equation}
    L(\boldsymbol{\Gamma}, \boldsymbol{\Phi})=L(\boldsymbol{\Gamma}, N_\theta(\boldsymbol{\Gamma}); \theta).
    \label{eq:unsupervised1}
\end{equation}
Note that the right hand side of \eqref{eq:unsupervised1} emphasizes that $L$ depends on the parameter $\theta$ given $\boldsymbol{\Gamma}$.

We collect massive channel data in a training data set $\mathcal{D}$
and formulate the unsupervised machine learning problem as
\begin{equation}
    \min_\theta \sum_{\boldsymbol{\Gamma} \in \mathcal{D}} L(\boldsymbol{\Gamma}, N_\theta(\boldsymbol{\Gamma}); \theta).
    \label{eq:ml_objective}
\end{equation}
In this way, we optimize the function which maps from any $\boldsymbol{\Gamma} \in \mathcal{D}$ to $\boldsymbol{\Phi}$.
This optimization process is called \emph{training}.
If the data set is general enough,
we would expect that a channel feature $\boldsymbol{\Gamma}' \notin \mathcal{D}$,
which, however, is \gls{iid} as channel features in $\mathcal{D}$,
can also be mapped to a good \gls{ris} configuration.
The performance evaluation of $L(\boldsymbol{\Gamma}', N_\theta(\boldsymbol{\Gamma}'))$ for $\boldsymbol{\Gamma}' \notin \mathcal{D}$ and a trained and fixed $N_\theta$ is called \emph{testing}.
\begin{remark}
Although $N_\theta$ is the same to any $\boldsymbol{\Gamma}$,
different $\boldsymbol{\Gamma}$ result in different $\boldsymbol{\Phi}$ with the same $N_\theta$.
Therefore, the obtained transmission power is not the ergodic power of all possible channels,
but is optimized for each particular channel.
\end{remark}
\begin{remark}
The training data is not exhaustive.
Therefore, to evaluate the performance of the trained model,
testing with $\boldsymbol{\Gamma}' \notin \mathcal{D}$ is mandatory.
Two keys to ensure the testing performance are 1) the model complexity and training process are reasonable enough to avoid overfitting, 2) the data in $\mathcal{D}$ is general enough such that $\boldsymbol{\Gamma}' \notin \mathcal{D}$ can be considered \gls{iid} as data in $\mathcal{D}$.
Since the distribution of channels can be very complicated 
(in particular when the channel is obtained with a complicated model, such as Ray-tracing, as applied in our work,
rather than sampled from a simple distribution, such as Rayleigh or Rician distribution),
massive data samples are required to ensure the testing performance.
\end{remark}


\subsection{Comparison of Machine Learning and Analytical Approaches}
While the correctness of analytical approaches is independent from the concrete input data,
there exists no closed-form solution for many difficult problems.
In these cases, either an approximation is applied to simplify the problem,
or an asymptotic iterative method is proposed.
Both of them result in a suboptimal performance.

On the other hand, a deep neural network can well approximate any continuous function in high dimensional space according to the universal approximation theorem~\cite{cybenko1989approximation}
in the sense that it is Kolmogorov-optimal approximants for markedly different
function classes with exponentially decaying approximation error in number of nonzero weights~\cite{elbrachter2021deep}.
Practically, the deep neural network has been successfully applied to approximate complicated mappings, such as from an image to its class in computation vision~\cite{ciregan2012multi}, or from a language to another in natural language processing~\cite{chowdhary2020natural} - we know such a mapping exists,
but it is hard to express with equations.
Motivated by these successes, we use the deep neural network to map the channel feature to the \gls{ris} configuration.
Although this mapping is difficult to obtain analytically,
it appears less complicated than the above-mentioned ones and therefore less risky.

Compare \eqref{eq:problem} and \eqref{eq:ml_objective},
we also notice a fundamental difference between analytical and machine learning approaches:
most analytical methods optimize $\boldsymbol{\Phi}$ itself,
the machine learning approach optimizes the function that maps from channel features $\boldsymbol{\Gamma}$ to \gls{ris} configuration $\boldsymbol{\Phi}$.
While the function optimization (training) is time-consuming,
the application of the function to a new channel feature without modifying the function itself (testing and deployment) requires significantly less computational power.
Moreover, the dedicated neural network architecture RISnet presented in Section~\ref{sec:architecture}
exploits the fact that the \gls{ris} antennas are homogeneous and therefore
can utilize the power of parallel computing,
as will be explained in detail in Section~\ref{sec:architecture}.
This is the reason that the machine learning approach requires less computational power in application than the analytical methods.
% the high complexity of the \gls{ris} optimization is due to the large number of \gls{ris} antennas,
% but the information processing of a single antenna is simple.
% Considering this, the information processing of layer~$i$ in RISnet is designed as
% \begin{equation}
%     N_i(\boldsymbol{\Gamma}) = P_i(Q_i(\gamma_1), Q_i(\gamma_2)\dots, Q_i(\gamma_N))
% \end{equation}
% where $P_i$ is an untrainable simple function (e.g., averaging),
% $Q_i$ is a trainable function for a single \gls{ris} antenna
% and $\gamma_n$ is the channel feature of \gls{ris} antenna~$n$.
% We note that computation of $Q_i(\gamma_n), n=1, 2, \dots, N$ can be parallelized since they are independent from each other.
% In this way, we can utilize the multiple thousands of cores in GPU or TPU.
% Computation of $P_i$ is fast because $P_i$ is simple.
% Although the computation of layer~$i+1$ requires output of layer~$i$,
% the number of layers is usually small (in our application, 8).

% On the contrary, widely-used analytical methods either cannot parallelize information processing of antennas (e.g., block coordinate descent (BCD)~\cite{Guo_Liang_Chen_Larsson_2020}) or propagation paths (e.g., space alternating generalized expectation-maximization (SAGE)~\cite{Fessler_Hero_1994}) because they depend on each other,
% or requires far more iterations than the number of layers in the neural network to converge (e.g., sequential convex approximation (SCA)~\cite{Zhu_Huang_Wang_Navaie_Ding_2021}).
% This difference makes the machine learning much more suitable for complicated and real-time optimization problems in the age of parallel computing.

To summarize, the machine learning approach has a higher potential of performance than analytical methods in specific problems because of its higher flexibility 
and requires less computational power and therefore is better scalable because the function is fixed in deployment and its ability to parallelize computation.
In Section~\ref{sec:results},
we will evaluate the performance of the proposed solution with both performance and computation complexity.

==> precoder.tex <==
\section{Machine Learning Solution for Joint Precoding and RIS Configuration}
\label{sec:ml}

\subsection{Objective Function and Framework of Unsupervised Learning}
\label{sec:objective}

The objective function defines how the neural network is optimized.
It should 1) enforce the quasi-degradation~\eqref{eq:quasi_degradation} since it is the prerequisite of applying the optimal precoding~\eqref{eq:optimal_precoding1} and \eqref{eq:optimal_precoding2},
2) minimize the transmission power in the quasi-degraded channel.
The objective function is therefore formulated as
\begin{equation}
    L = \log \left(1 + \text{ReLU} \left(Q - \frac{\norm{\bh_1}^2}{\norm{\bh_2}^2} \right)\right) + \epsilon P,
    \label{eq:objective}
\end{equation}
where the first term is the penalty if the channel is not quasi-degraded
and the second term is the transmission power,
the constant factor $\epsilon$ is chosen to balance the effort to make all channels quasi-degraded and to minimize the transmission power.

We define the neural network as $N_\theta$,
which is a function parameterized by $\theta$ and
maps from the channel feature $\boldsymbol{\Gamma}$,
which will be defined in Section~\ref{sec:feature_definition},
to the \gls{ris} phase shifts $\boldsymbol{\Phi}$,
i.e., $\boldsymbol{\Phi} = N_\theta(\boldsymbol{\Gamma}).$
With the optimal precoding for quasi-degraded channels presented in Section~\ref{sec:quasi},
our objective function $L$
is fully determined by the channel feature $\boldsymbol{\Gamma}$,
and the \gls{ris} configuration $\boldsymbol{\Phi}$.
We can write the objective as $ L(\boldsymbol{\Gamma}, \boldsymbol{\Phi})=L(\boldsymbol{\Gamma}, N_\theta(\boldsymbol{\Gamma}); \theta).$
Note that the right hand side of the equation emphasizes that $L$ depends on the parameter $\theta$ given $\boldsymbol{\Gamma}$.

We collect massive channel data in a training data set $\mathcal{D}$
and formulate the unsupervised machine learning problem as
\begin{equation}
    \min_\theta \sum_{\boldsymbol{\Gamma} \in \mathcal{D}} L(\boldsymbol{\Gamma}, N_\theta(\boldsymbol{\Gamma}); \theta).
    \label{eq:ml_objective}
\end{equation}
In this way, we optimize the function which maps from any $\boldsymbol{\Gamma} \in \mathcal{D}$ to $\boldsymbol{\Phi}$.
This optimization process is called \emph{training}.
If the data set is general enough,
we would expect that a channel feature $\boldsymbol{\Gamma}' \notin \mathcal{D}$,
which, however, is \gls{iid} as channel features in $\mathcal{D}$,
can also be mapped to a good \gls{ris} configuration.
The performance evaluation of $L(\boldsymbol{\Gamma}', N_\theta(\boldsymbol{\Gamma}'))$ for $\boldsymbol{\Gamma}' \notin \mathcal{D}$ and a trained and fixed $N_\theta$ is called \emph{testing}.

\subsection{Channel Features}
\label{sec:feature_definition}

We assume that $\mathbf{H}$ is constant because both \gls{bs} and \gls{ris} are fixed.
The neural network requires both $\bh_{dk}$ and $\bh_{rk}, k=1, 2$ to compute $\bPhi$.
The \gls{ris} optimization problem is complicated mainly because of the large number of \gls{ris} antennas.
However, the way that one single \gls{ris} antenna contributes to the overall channel is the same,
i.e., the \gls{ris} antennas are homogeneous.
Motivated by this fact,
we apply the same information processing for every \gls{ris} antenna in one layer of the multi-layer deep neural network.
This requires that the input of the deep neural network, i.e., the channel feature,
should be a stack of channel features per \gls{ris} antenna.
While this is straightforward for $\bh_{rk}^H$ 
because column~$n$ of $\bh_{rk}^H$ is the channel gain from \gls{ris} antenna~$n$ to user~$k$,
it is difficult for $\bh_{dk}^H$ since $\bh_{dk}^H$ is the direct channel from \gls{ris} to user~$k$.
Therefore, we apply the following trick:
\begin{equation}
    \bh_k^H=\bh_{rk}^H \bPhi \bH + \bh_{dk}^H = (\bh_{rk}^H \bPhi + \bj^H_k)\bH,
    \label{eq:}
\end{equation}
where we define $\bj^H_k = \bh_{dk}^H\bH^+$ with $\bH^+$ being the pseudo-inverse of $\bH$.
Column~$n$ of vector $\bj_k^H \in \mathbb{C}^{1\times N}$ can then be mapped to \gls{ris} antenna~$n$ unambiguously.
The channel feature $\boldsymbol{\Gamma}$ is defined as
\begin{equation}
\begin{aligned}
    \bs{\Gamma} = ( & |\bh^H_{r1}|; \arg(\bh^H_{r1}); |\bj^H_{1}|; \arg(\bj^H_{1})\\
    & |\bh^H_{r2}|; \arg(\bh^H_{r2}); |\bj^H_{2}|; \arg(\bj^H_{2})),
\end{aligned}
\label{eq:feature_definition}
\end{equation}
where the semicolon indicates a new row of the matrix.
$\bs{\Gamma}$ has a shape of $8\times N$.
Column~$n$ of $\bs{\Gamma}$ is the channel feature of \gls{ris} antenna~$n$.

% \subsection{Objective Functions}

% Our objective function~$f$ in \eqref{eq:problem} is a function of channels $\mb{G}$ and $\mb{D}$, 
% \gls{ris} phase shifts $\bs{\Phi}$ and \gls{bs} precoding $\mb{V}$. 
% When $\bs{\Phi}$ is determined, 
% $\mb{V}$ can be computed with either \gls{mmse} precoder or \gls{wmmse} precoder as described in Section~\ref{sec:precoder},
% which are denoted as $\mb{V}_{\text{MMSE}}(\mb{G}, \mb{D}, \bs{\Phi})$ and $\mb{V}_{\text{WMMSE}}(\mb{G}, \mb{D}, \bs{\Phi})$, respectively.
% It is to note that $\mb{V}_{\text{MMSE}}$ is a differentiable function but $\mb{V}_{\text{WMMSE}}$ is not differentiable.

% Since $f$ is a function of $\mb{G}$, $\mb{D}$, $\bs{\Phi}$ and $\mb{V}$,
% we can express $f$ as $f(\mb{G}, \mb{D}, \bs{\Phi}, \mb{V})$. Therefore, for \gls{mmse} precoding, the objective function is
% \begin{equation}
% \begin{aligned}
%     f\bigg(& \mb{G}, \mb{D}, \exp\big(j\p(\mb{G}, \mb{D})\big), \\
%     & \mb{V}_{\text{MMSE}}\Big(\mb{G}, \mb{D}, \exp\big(j\p(\mb{G}, \mb{D})\big)\Big)\bigg).
% \end{aligned}
% \label{eq:objective_mmse}
% \end{equation}

% For \gls{wmmse} precoding, the objective function is
% \begin{equation}
% \begin{aligned}
%     f\bigg(& \mb{G}, \mb{D}, \exp\big(j\p(\mb{G}, \mb{D})\big), \\
%     & \mb{V}_{\text{WMMSE}}\Big(\mb{G}, \mb{D}, \exp\big(j\bs{\Psi}_{\bar{\theta}}(\mb{G}, \mb{D})\big)\Big)\bigg).
% \end{aligned}
% \label{eq:objective_wmmse}
% \end{equation}
% Please note that $\bs{\Psi}_{\bar{\theta}}$ in \eqref{eq:objective_wmmse} is untrainable, i.e., $\bar{\theta}$ is given and $\bs{\Psi}_{\bar{\theta}}(\mb{G}, \mb{D})$ is a constant.
% Therefore, we do not need to compute the derivative of $\mb{V}_{\text{WMMSE}}$ since it does not contain trainable variable $\theta$.

% We can then compute $\frac{\partial f}{\partial \theta}$ to do gradient ascent to optimize $\p$ such that $f$ is maximized for both \eqref{eq:objective_mmse} and \eqref{eq:objective_wmmse}.
% The Adam optimizer~\cite{kingma2014adam} is chosen to perform the optimization.
